RangeDet:In Defense of Range View for LiDAR-based 3D Object Detection

In this paper, we propose an anchor-free single-stage LiDAR-based 3D object detector -- RangeDet. The most notable difference with previous works is that our method is purely based on the range view representation. Compared with the commonly used voxelized or Bird's Eye View (BEV) representations, the range view representation is more compact and without quantization error. Although there are works adopting it for semantic segmentation, its performance in object detection is largely behind voxelized or BEV counterparts. We first analyze the existing range-view-based methods and find two issues overlooked by previous works: 1) the scale variation between nearby and far away objects; 2) the inconsistency between the 2D range image coordinates used in feature extraction and the 3D Cartesian coordinates used in output. Then we deliberately design three components to address these issues in our RangeDet. We test our RangeDet in the large-scale Waymo Open Dataset (WOD). Our best model achieves 72.9/75.9/65.8 3D AP on vehicle/pedestrian/cyclist. These results outperform other range-view-based methods by a large margin (~20 3D AP in vehicle detection), and are overall comparable with the state-of-the-art multi-view-based methods. Codes will be public.

==> point_op.tex <==
In this section, we compare Meta-Kernel with some typical point-based operator: PointNet~\cite{pointnet}, DGCNN~\cite{dgcnn}, Continuous Conv~\cite{cc}.
\par
\textbf{Motivation.} The motivations of point-based operators are mainly lie in extract effictive features directly from irregular point clouds.
Our Meta-Kernel is aimmed to extract features containing 3D geometric information efficiently and densely from 2D range image.
So Meta-Kernel is more like 2D convolution with fixed $n \times n$ neighbourhood other than a point-based operator defined on unordered point set.
\textbf{Application scenarios.} Typical point-based operators usually need to select key points and find neighbours.
For example, Farthest Point Sampling (FPS) and Ball Query (BQ) are necessary components of 3D detectors using point-based operators.
The time complexity of FPS and BQ are $O(n^2)$ as the number of key points usually proportional to the number of all points.
It is not efficient enough to process large scale point clouds in the autonomous driving scenario.
For example, the inference time of PointRCNN~\cite{pointrcnn} with point cloud from a complete KITTI frame is xx ms.
So point-based operators are usually apply to indoor scenes, while the efficency of Meta-Kernel enable dense feature extraction in autonomous driving scenario, where the number of points per frame is usually greater than 10K.

==> tables/ablation_table.tex <==
\begin{table*}[t]
	\footnotesize 
	\begin{center}
		\scalebox{0.975}{
			\begin{tabular}{c|ccccc|cccc|cccc}
				\toprule
				\multirow{2}{*}{} &\multirow{2}{*}{\shortstack[1]{Meta-\\Kernel}} & \multirow{2}{*}{RCP} & \multirow{2}{*}{\shortstack[1]{IoU\\Prediction}} & \multirow{2}{*}{WNMS} & \multirow{2}{*}{DA} & 			
				\multicolumn{4}{c|}{3D AP (IoU=0.7)} & \multicolumn{4}{c}{BEV AP (IoU=0.7)} \\
				&&&&&&Overall & 0 - 30 & 30 - 50 & 50 - inf & Overall & 0 - 30 & 30 - 50 & 50 - inf\\
				\midrule
				A1& &  &  &  & &53.39 & 73.02 & 48.79 & 28.14 & 70.45 & 86.22 & 68.45 & 51.90 \\
				A2&\checkmark &  & &  &  & 56.58 & 76.11 & 54.29& 32.53 & 74.89 & 88.14 & 71.43 & 57.55\\
				A3&&\checkmark   & &  &  & 58.37 & 78.66 & 50.40& 32.35 & 78.02 & 90.71 & 73.13 & 62.23\\
				A4&\checkmark & \checkmark &  & &  & 61.05 & 80.11 & 54.59 & 35.95 & 80.65 & 92.12 & 78.20 & 66.58\\
				A5&\checkmark & \checkmark & \checkmark &  & &63.86 & 82.65& 60.01 & 39.85 & 82.03 & 92.90 &80.17 & 68.56 \\
				A6&\checkmark & \checkmark & \checkmark & \checkmark && 69.00 & {86.89} & {66.16} & 45.81 & 85.48 & 93.62 & 82.17 & 72.97\\
				A6& & \checkmark & \checkmark & \checkmark && 67.54 & {86.49} & {62.86} & 41.67 & 82.25 & 93.20 & 80.87 & 68.38\\
				A7&\checkmark &  & \checkmark & \checkmark & &64.35 & 82.60 & 60.11 & 39.91 & 77.33 & 89.19 & 75.69 & 61.33\\
				A8& &  & \checkmark & \checkmark & & 61.08 & 81.78 & 58.07 & 36.22 & 76.20 & 88.78 & 72.31 & 58.94\\
				% A9&\checkmark & \checkmark & \checkmark & \checkmark & \checkmark & 72.85 & {87.96} & {69.03} & 48.88 & 86.94 & 94.35 & 85.66 & 77.01\\
				 \bottomrule
			\end{tabular}
		}	
	\end{center}
	\vspace{-2mm}
	\caption{Ablation of our components on vehicle detection. DA stands for data augmentation.}
	\label{tab:ablation}
	\vspace{-3mm}
\end{table*}

==> tables/ped_table.tex <==
\begin{table*}[h]
	\footnotesize 
	\begin{center}
		\scalebox{0.975}{
			\begin{tabular}{c||c|cccc|cccc}
				\toprule
				\multirow{2}{*}{Method} & \multirow{2}{*}{View} & 			
				\multicolumn{4}{c|}{3D AP (IoU=0.5)} & \multicolumn{4}{c}{BEV AP (IoU=0.5)} \\
				&&Overall & 0m - 30m & 30m - 50m & 50m - inf & Overall & 0m - 30m & 30m - 50m & 50m - inf\\
				
				\midrule
				PointPillars$\ast$~\cite{pointpillar} & BEV & 59.25 & 67.99 & 57.01 & 41.29 & 68.57 & 75.02 & 67.11 & 53.86\\
				PointPillars$\dag$~\cite{pointpillar} & BEV & 60.0 & 68.9 & 57.6 & 46.0 & 68.7 & 75.0 & 66.6 & 58.7\\
				DynVox\cite{mvf} & BEV & 60.83 & 69.76 & 58.43 & 42.06 & 70.25 & 77.01 & 68.96 & 54.15\\
				MVF~\cite{mvf} & BEV + RV & 65.33 & 72.51 & 63.35 & 50.62 & 74.38 & 80.01 & 72.98 & 62.51\\
                PillarBased~\cite{pillarbased} & BEV + CV & \best{72.51} & \best{79.34} & \best{72.14} & \second{56.77} & \best{78.53} & \best{83.56} & \best{78.7} & \second{65.86}\\
                \midrule
				LaserNet~\cite{lasernet} & RV & 63.4 & 73.47 & 61.55 & 42.69 & 70.01 & 78.24 & 69.47 & 52.68\\
                \midrule
				Ours & RV & \second{70.76} & \second{77.77} & \second{70.97} & \best{59.58} & \second{76.95} & \second{82.69} & \second{77.68} & \best{69.32}\\
				\bottomrule
			\end{tabular}
		}	
	\end{center}
	\caption{Results on pedestrian evaluated on WOD validation split. The meaning of terminologies and notations in this table is the same as in Table \ref{tab:sota}. The best result and the second result are marked in \best{red} and \second{blue}, respectively.}
	\label{tab:ped_sota}
	\vspace{-3mm}
\end{table*}

==> tables/point_op_cat.tex <==
\begin{table}[!h]
	\small 
  \begin{center}
    \resizebox{0.95\linewidth}{!}{
		% \scalebox{0.975}{
			\begin{tabular}{c|ccccc}
				\toprule
				\multirow{2}{*}{Method} &  			
				\multicolumn{4}{c}{3D AP on Vehicle (IoU=0.7)}\\
				&Overall & 0 - 30 & 30 - 50 & 50 - inf\\
                \midrule
        PointNet-RV-Cat~\cite{pointnet} &  64.74 & 85.48 & 60.86 & 40.48\\
        EdgeConv-RV-Cat~\cite{dgcnn} &  67.28 & 85.82 & 62.66 & 42.90\\
        RandLA-RV-Cat~\cite{randla} &  67.39 & 85.91 & 62.50 & 43.21\\
				\bottomrule
			\end{tabular}
		}	
	\end{center}
	\vspace{-2mm}
  \caption{Performance of point-based operators in RV. Suffix ``Cat'' means that the aggregation step in the operator is replaced by concatenation. Continuous Conv and RSConv have a very similar formulation to Meta-Kernel when their aggregation step is replaced by concatenation, so we do not list them in this table.}
	\label{tab:point_op_cat}
	\vspace{-2mm}
\end{table}
